Tolerant Bipartiteness Testing in Dense Graphs

Bipartite testing has been a central problem in the area of property testing since its inception in the seminal work of Goldreich, Goldwasser and Ron [FOCS'96 and JACM'98]. Though the non-tolerant version of bipartite testing has been extensively studied in the literature, the tolerant variant is not well understood. In this paper, we consider the following version of tolerant bipartite testing: Given a parameter $\varepsilon \in (0,1)$ and access to the adjacency matrix of a graph $G$, we can decide whether $G$ is $\varepsilon$-close to being bipartite or $G$ is at least $(2+\Omega(1))\varepsilon$-far from being bipartite, by performing $\widetilde{\mathcal{O}}\left(\frac{1}{\varepsilon ^3}\right)$ queries and in $2^{\widetilde{\mathcal{O}}(1/\varepsilon)}$ time. This improves upon the state-of-the-art query and time complexities of this problem of $\widetilde{\mathcal{O}}\left(\frac{1}{\varepsilon ^6}\right)$ and $2^{\widetilde{\mathcal{O}}(1/\varepsilon^2)}$, respectively, from the work of Alon, Fernandez de la Vega, Kannan and Karpinski (STOC'02 and JCSS'03), where $\widetilde{\mathcal{O}}(\cdot)$ hides a factor polynomial in $\log \frac{1}{\varepsilon}$.

==> intro.tex <==
\section{??}

A \emph{bipartition} of (the vertices of) a graph $G$ is a function $f:V(G)\rightarrow \{L,R\}$~\footnote{ $L$ and $R$ denote left and right, respectively.}. The \emph{bipartite} distance of  graph $G$ with respect to bipartition $f$ is denoted and defined as 
$$d_{bip}(G,f)=\sum_{v\in V:f(v)=L}|N(v)\cap f^{-1}(L)|+ \sum_{v\in V:f(v)=R}|N(v)\cap f^{-1}(R)|$$

Informally speaking, $d_{bip}(G,f)$ measures the farness of the graph $G$ from beign bipartite with respect to a bipartition $f$. The \emph{bipartite distance} of graph $G$ is defined as the minimum bipartite distance of $G$ over all possible bipartitions $f$, that is, 
$$d_{bip}(G)=\min_{f}d_{bip}(G,f).$$
%\complain{Need to write something about the query model and an informal description of our result.}

It is interesting to note that bipartite distance is deeply connected to the size of maxcut. Namely, we have the following:
$$\size{MaxCut(G)}= \size{E(G)} - d_{bip}(G) $$

Thus in order to estimate the size of maxcut, it is enough to estimate both the  number of edges as well as the bipartite distance of the graph. Since $G$ is dense, we can estimate $E(G)$ with only $O(\frac{1}{\eps^3})$ many queries.


\begin{obs}[Folklore]
Given any graph $G$ on $n$ vertices, the size of the edge set $E(G)$ can be estimated within an additive $\eps n^2$ error, with probability at least $3/4$, using $O(\frac{1}{\eps^3})$ many adjacency queries to $G$. Note that time and sample complexity of the algorithm will also be $O\left( \frac{1}{\eps^{3}}\right)$.
\end{obs}

Now we come to the main technical result of this paper. We essentially prove that $d_{bip}(G)$ can be estimated by only performing $\widetilde{O}(\frac{1}{\eps^4})$ many adjacency queries, thereby estimating the size of $MaxCut(G)$.


%\textcolor{blue}{add sample complexity, time complexity}

\begin{theo}
Given a graph $G$ on $n$ vertices and a proximity parameter $\eps \in [0,1]$, there exists an algorithm that samples $\widetilde{O}(\frac{1}{\eps^3})$ many vertices, performs $\widetilde{O}(\frac{1}{\eps^4})$ many adjacency queries and in time $2^{\widetilde{O}(\frac{1}{\eps})}$, outputs a number $\beta$ such that
$$
    d_{bip}(G) -\eps n^{2} \leq \beta \leq d_{bip}(G) + \eps n^{2} 
$$
\end{theo}

Since from the seminal result of Rubinfeld, Parnas and Ron??, we know that estimating the bipartite distance of $G$ is equivalent to deciding the tolerant version of the problem with an extra poly-logarithmic complexity, we will be essentially working with the tolerant version of bipartite distance of $G$, as follows:

%The result is formally stated as follows.
\begin{theo}\label{theo:main}
There exists an algorithm that given adjacency query access to a graph $G$ with $n$ vertices and a parameter $\eps \in \left[0,1\right]$, decides whether $d_{bip}(G) \leq \eps n^2$ or $d_{bip}(G) \geq \spcl \eps n^2$ by sampling $\widetilde{O}(\frac{1}{\eps})$ many vertices in $2^{\widetilde{O}(\frac{1}{\eps})}$ time, using $\tOh(\frac{1}{\eps^4})$ many queries to the adjacency matrix of $G$. 
\end{theo}


\subsection{Overview of our proof}\label{sub:over}
\subsection{Related work}
\subsection{Organization of the paper}
\subsection{Notation}
For us, $o_{\eps}(1)$ represents $1- \eps^c$ for some suitable constant $c$.

==> prelim.tex <==
\section{Preliminaries}\label{sec:pre}
\comments{Recall the definition of bipartition of the vertices of the graph $G$, that is, it refers to a function $f:V(G)\rightarrow \{L,R\}$. Similarly, we can extend the definition of the bipartition of any subset $U \subseteq V(G)$ as $f\mid_U$, that is, function $f$ restricted to $U$. For simplicity of presentation, we sometime denote a bipartition $f\mid_U$ for $U\subseteq V(G)$ as a pair $\left(U_L,U_R\right)$, where $U_L$ and $U_R$ denote the vertices that $f$ ($f\mid_U$) maps to $L$ and $R$, respectively. We denote a bipartition as a function as well as a pair (as described above) interchangeably, and it will be clear from the context.}

%\complain{Need to define decider}


